Reasoning about Polymorphic Manifest Contracts

Manifest contract calculi, which integrate cast-based dynamic contract checking and refinement type systems, have been studied as foundations for hybrid contract checking. In this article, we study techniques to reasoning about a polymorphic manifest contract calculus, including a few program transformations related to static contract verification. We first define a polymorphic manifest contract calculus $\mathrm{F}_{H}$, which is much simpler than a previously studied one with delayed substitution, and a logical relation for it and prove that the logical relation is sound with respect to contextual equivalence. Next, we show that the upcast elimination property, which has been studied as correctness of subtyping-based static cast verification, holds for $\mathrm{F}_{H}$. More specifically, we give a subtyping relation (which is not part of the calculus) for $\mathrm{F}_{H}$ types and prove that a term obtained by eliminating upcasts---casts from one type to a supertype of it---is logically related and so contextually equivalent to the original one. We also justify two other program transformations for casts: selfification and static cast decomposition, which help upcast elimination. A challenge is that, due to the subsumption-free approach to manifest contracts, these program transformations do not always preserve well-typedness of terms. To address it, the logical relation and contextual equivalence in this work are defined as semityped relations: only one side of the relations is required to be well typed and the other side may be ill typed.

==> sections/upcast_elim.tex <==
\section{Upcast Elimination}
\label{sec:upcast-elim}

We introduce subtyping for {\fhfix} and show that an upcast and an identity
function are contextual equivalent by using the logical relation given in
\sect{logical_relation}.

 \subsection{Subtyping}

 \begin{fhfigure*}[t!]
  \begin{flushleft}
   \framebox{$\Gamma  \vdash  \ottnt{T_{{\mathrm{1}}}}  \ottsym{<:}  \ottnt{T_{{\mathrm{2}}}}$} \quad {\bf{Subtyping Rules}}
  \end{flushleft}

  \begin{center}
   $\ottdruleSXXBase{}$ \hfil
   $\ottdruleSXXTVar{}$ \hfil
   $\ottdruleSXXForall{}$ \\[1.5ex]
   $\ottdruleSXXFun{}$ \\[1.5ex]
   $\ottdruleSXXRefineL{}$
   $\ottdruleSXXRefineR{}$
  \end{center}

  \vspace{1em}
  \begin{flushleft}
   \framebox{$\Gamma  \models  \ottnt{e}$} \quad {\bf{Satisfaction Rule}}
  \end{flushleft}

  \begin{center}
   $\ottdruleSatis{}$
  \end{center}
  \caption{Subtyping rules.}
  \label{fig:subtype}
 \end{fhfigure*}

 \fig{subtype} shows subtyping rules, which are similar to Belo et
 al.~\cite{Belo/Greenberg/Igarashi/Pierce_2011_ESOP} except that we decompose
 the subtyping rule for refinement types into two simple rules.
 \TS{Knowles and Flanagan don't need substitution of cast applications for arguments in the case of function types.  We have to note it?}
 %
 Subtyping judgment $\Gamma  \vdash  \ottnt{T_{{\mathrm{1}}}}  \ottsym{<:}  \ottnt{T_{{\mathrm{2}}}}$ takes typing context $\Gamma$ for
 checking refinements in $\ottnt{T_{{\mathrm{2}}}}$.
 %
 Base types and type variables can be subtypes of only themselves
 (\Sub{Base} and \Sub{TVar}).
 %
 \Sub{Forall} checks that body types of universal types are in subtyping.
 %
 As for function types, subtyping is contravariant on the domain types
 and covariant on the codomain types \Sub{Fun}.
 %
 The subtyping judgment on codomain types assumes that the type of argument
 $\mathit{x}$ is $\ottnt{T_{{\mathrm{21}}}}$, a subtype of the other domain type $\ottnt{T_{{\mathrm{11}}}}$, but
 codomain type $\ottnt{T_{{\mathrm{12}}}}$ refers to $\mathit{x}$ as $\ottnt{T_{{\mathrm{11}}}}$.
 %
 Since the type system of {\fhfix} does not allow subsumption for subtyping, we
 force $\mathit{x}$ to be of $\ottnt{T_{{\mathrm{11}}}}$ by inserting an upcast, which can be
 eliminated after showing upcast elimination.
 %
 We can refine a subtype furthermore \Sub{RefineL}.
 %
 By contrast, a supertype can be refined if we can prove that any value of the
 subtype satisfies the refinement \Sub{RefineR}.
 %
 Term $\ottnt{e}$ is satisfied under $\Gamma$ ($\Gamma  \models  \ottnt{e}$) if,
 for any closing substitution $\sigma$ that respects $\Gamma$,
 $ \sigma  (  \ottnt{e}  ) $ evaluates to $ \mathsf{true} $.
 %
 \Sub{RefineR} also inserts an upcast since
 satisfaction assumes that the type of $\mathit{x}$ is $\ottnt{T_{{\mathrm{1}}}}$ but
 $\ottnt{e}$ refers to it as $\ottnt{T_{{\mathrm{2}}}}$.
 
 \subsection{Upcast Elimination}

 We show that an upcast and an identity function are logically related; then
 soundness of the logical relation implies that they are contextually
 equivalent.

% \begin{prop}{fh-ciu-subterm-eval}
%  If
%  $\ottnt{e}  \longrightarrow^{\ast}  \ottnt{v}$ and
%  $\emptyset  \vdash  \ottnt{e'} \, [  \ottnt{v}  \ottsym{/}  \mathit{x}  ]  \ottsym{:}  \ottnt{T}$,
%  then
%  $\emptyset  \vdash  \ottnt{e'} \, [  \ottnt{v}  \ottsym{/}  \mathit{x}  ] \, =_\mathsf{ciu} \, \ottnt{e'} \, [  \ottnt{e}  \ottsym{/}  \mathit{x}  ]  \ottsym{:}  \ottnt{T}$.

%  \proof

%  We show that, for any $\ottnt{E}^\ottnt{S}$ and $\ottnt{T'}$ such that
%  $\emptyset  \vdash  \ottnt{E}^\ottnt{S}  \ottsym{:}  \ottsym{(}  \emptyset  \vdash  \ottnt{e'} \, [  \ottnt{v}  \ottsym{/}  \mathit{x}  ]  \ottsym{:}  \ottnt{T}  \ottsym{)}  \mathrel{\circ\hspace{-.4em}\rightarrow}  \ottnt{T'}$,
%  \[
%   \ottnt{E}^\ottnt{S}  [  \ottnt{e'} \, [  \ottnt{v}  \ottsym{/}  \mathit{x}  ]  ]  \Downarrow  \ottnt{E}^\ottnt{S}  [  \ottnt{e'} \, [  \ottnt{e}  \ottsym{/}  \mathit{x}  ]  ].
%  \]
%  %
%  Since $\emptyset  \vdash  \ottnt{E}^\ottnt{S}  [  \ottnt{e'} \, [  \ottnt{v}  \ottsym{/}  \mathit{x}  ]  ]  \ottsym{:}  \ottnt{T'}$,
%  we have $\emptyset  \vdash  \ottnt{E}^\ottnt{S}  [  \ottnt{e'} \, [  \ottnt{v}  \ottsym{/}  \mathit{x}  ]  ] \,  \mathrel{ \simeq }  \, \ottnt{E}^\ottnt{S}  [  \ottnt{e'} \, [  \ottnt{v}  \ottsym{/}  \mathit{x}  ]  ]  \ottsym{:}  \ottnt{T'}$
%  by Parametricity (\prop:ref{fh-lr-param}).
%  %
%  Thus,
%  (1) $ \ottnt{E}^\ottnt{S}  [  \ottnt{e'} \, [  \ottnt{v}  \ottsym{/}  \mathit{x}  ]  ]  \downarrow $ or
%  (2) $ \ottnt{E}^\ottnt{S}  [  \ottnt{e'} \, [  \ottnt{v}  \ottsym{/}  \mathit{x}  ]  ]  \, \mathord{\Uparrow}  \ell $ for some $\ell$.
%  %
%  In the case (1), $ \ottnt{E}^\ottnt{S}  [  \ottnt{e'} \, [  \ottnt{e}  \ottsym{/}  \mathit{x}  ]  ]  \downarrow $
%  by Cotermination (\prop:ref{fh-coterm-true}).
%  %
%  In the case (2), we can show that $ \ottnt{E}^\ottnt{S}  [  \ottnt{e'} \, [  \ottnt{e}  \ottsym{/}  \mathit{x}  ]  ]  \, \mathord{\Uparrow}  \ell $
%  in a similar way to Cotermination.
% \end{prop}

\begin{prop}{fh-elim-upcast-aux}
 If
 $\Gamma  \vdash  \ottnt{T_{{\mathrm{1}}}}$ and
 $\Gamma  \vdash  \ottnt{T_{{\mathrm{2}}}}$ and
 $\Gamma  \vdash  \ottnt{T_{{\mathrm{1}}}}  \ottsym{<:}  \ottnt{T_{{\mathrm{2}}}}$ and
 $\Gamma  \vdash  \theta  \ottsym{;}  \delta$,
 then
 $  \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T_{{\mathrm{1}}}}  \Rightarrow  \ottnt{T_{{\mathrm{2}}}}  \rangle   ^{ \ell }   )   )   \simeq_{\mathtt{v} }   \theta_{{\mathrm{2}}}  (   \delta_{{\mathrm{2}}}  (    \lambda    \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{1}}}}  .  \mathit{x}   )   )    \ottsym{:}   \ottnt{T_{{\mathrm{1}}}}  \rightarrow  \ottnt{T_{{\mathrm{2}}}} ;  \theta ;  \delta $.

 \proof

 By induction on $\Gamma  \vdash  \ottnt{T_{{\mathrm{1}}}}  \ottsym{<:}  \ottnt{T_{{\mathrm{2}}}}$.
 %
 It suffices to show that,
 for any $\ottnt{v_{{\mathrm{1}}}}$ and $\ottnt{v_{{\mathrm{2}}}}$ such that $ \ottnt{v_{{\mathrm{1}}}}  \simeq_{\mathtt{v} }  \ottnt{v_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T_{{\mathrm{1}}}} ;  \theta ;  \delta $,
 \[
    \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T_{{\mathrm{1}}}}  \Rightarrow  \ottnt{T_{{\mathrm{2}}}}  \rangle   ^{ \ell }   )   )  \, \ottnt{v_{{\mathrm{1}}}}  \simeq_{\mathtt{e} }  \ottnt{v_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T_{{\mathrm{2}}}} ;  \theta ;  \delta .
 \]
 %
 We proceed by case analysis on the rule applied last to derive
 $\Gamma  \vdash  \ottnt{T_{{\mathrm{1}}}}  \ottsym{<:}  \ottnt{T_{{\mathrm{2}}}}$.
 %
 \begin{itemize}
  \case \Sub{Base}: Obvious
   since $\langle  \ottnt{B}  \Rightarrow  \ottnt{B}  \rangle   ^{ \ell }  \, \ottnt{v_{{\mathrm{1}}}}  \longrightarrow  \ottnt{v_{{\mathrm{1}}}}$ and $ \ottnt{v_{{\mathrm{1}}}}  \simeq_{\mathtt{v} }  \ottnt{v_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{B} ;  \theta ;  \delta $.

  \case \Sub{TVar}:
   %
   We are given $\Gamma  \vdash  \alpha  \ottsym{<:}  \alpha$.
   %
   Since $\Gamma  \vdash  \alpha$ and $\Gamma  \vdash  \theta  \ottsym{;}  \delta$,
   there exists some $\ottnt{r'}$, $\ottnt{T'_{{\mathrm{1}}}}$, and $\ottnt{T'_{{\mathrm{2}}}}$ such that
   $ \theta  (  \alpha  ) = (  \ottnt{r'} ,  \ottnt{T'_{{\mathrm{1}}}} ,  \ottnt{T'_{{\mathrm{2}}}}  ) $.
   %
   Since $ \ottnt{v_{{\mathrm{1}}}}  \simeq_{\mathtt{v} }  \ottnt{v_{{\mathrm{2}}}}   \ottsym{:}   \alpha ;  \theta ;  \delta $, we have $\ottsym{(}  \ottnt{v_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{v_{{\mathrm{2}}}}  \ottsym{)} \, \in \, \ottnt{r'}$.
   %
   Since $\ottnt{r'} \, \in \,  \mathsf{VRel}  (  \ottnt{T'_{{\mathrm{1}}}} ,  \ottnt{T'_{{\mathrm{2}}}}  ) $,
   there exists some $\ottnt{v'_{{\mathrm{1}}}}$ such that
   $\langle  \ottnt{T'_{{\mathrm{1}}}}  \Rightarrow  \ottnt{T'_{{\mathrm{1}}}}  \rangle   ^{ \ell }  \, \ottnt{v_{{\mathrm{1}}}}  \longrightarrow^{\ast}  \ottnt{v'_{{\mathrm{1}}}}$ and $\ottsym{(}  \ottnt{v'_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{v_{{\mathrm{2}}}}  \ottsym{)} \, \in \, \ottnt{r'}$.
   %
   Thus, $ \ottnt{v'_{{\mathrm{1}}}}  \simeq_{\mathtt{v} }  \ottnt{v_{{\mathrm{2}}}}   \ottsym{:}   \alpha ;  \theta ;  \delta $.

  \case \Sub{Fun}:
   %
   We are given $\Gamma  \vdash   \mathit{x} \mathord{:} \ottnt{T_{{\mathrm{11}}}} \rightarrow \ottnt{T_{{\mathrm{12}}}}   \ottsym{<:}   \mathit{x} \mathord{:} \ottnt{T_{{\mathrm{21}}}} \rightarrow \ottnt{T_{{\mathrm{22}}}} $.
   %
   By inversion, we have
   $\Gamma  \vdash  \ottnt{T_{{\mathrm{21}}}}  \ottsym{<:}  \ottnt{T_{{\mathrm{11}}}}$ and $ \Gamma  ,  \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{21}}}}   \vdash  \ottnt{T_{{\mathrm{12}}}} \, [  \langle  \ottnt{T_{{\mathrm{21}}}}  \Rightarrow  \ottnt{T_{{\mathrm{11}}}}  \rangle   ^{ \ell }  \, \mathit{x}  \ottsym{/}  \mathit{x}  ]  \ottsym{<:}  \ottnt{T_{{\mathrm{22}}}}$.
   %
   Without loss of generality, we can suppose that $\mathit{x} \, \notin \,  \mathit{dom}  (  \delta  ) $.
   %
   By \E{Red}/\R{Fun},
   \[\begin{array}{l}
     \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle   \mathit{x} \mathord{:} \ottnt{T_{{\mathrm{11}}}} \rightarrow \ottnt{T_{{\mathrm{12}}}}   \Rightarrow   \mathit{x} \mathord{:} \ottnt{T_{{\mathrm{21}}}} \rightarrow \ottnt{T_{{\mathrm{22}}}}   \rangle   ^{ \ell }   )   )  \, \ottnt{v_{{\mathrm{1}}}}  \longrightarrow  \\ \quad
      \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (    \lambda    \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{21}}}}  .   \mathsf{let}  ~  \mathit{y}  \mathord{:}  \ottnt{T_{{\mathrm{11}}}}  \equal  \langle  \ottnt{T_{{\mathrm{21}}}}  \Rightarrow  \ottnt{T_{{\mathrm{11}}}}  \rangle   ^{ \ell }  \, \mathit{x}  ~ \ottliteralin ~  \langle  \ottnt{T_{{\mathrm{12}}}} \, [  \mathit{y}  \ottsym{/}  \mathit{x}  ]  \Rightarrow  \ottnt{T_{{\mathrm{22}}}}  \rangle   ^{ \ell }   \, \ottsym{(}  \ottnt{v_{{\mathrm{1}}}} \, \mathit{y}  \ottsym{)}   )   ) 
     \end{array}\]
   for a fresh variable $\mathit{y}$.
   %
   By definition, it suffices to show that,
   for any $\ottnt{v'_{{\mathrm{1}}}}$ and $\ottnt{v'_{{\mathrm{2}}}}$ such that $ \ottnt{v'_{{\mathrm{1}}}}  \simeq_{\mathtt{v} }  \ottnt{v'_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T_{{\mathrm{21}}}} ;  \theta ;  \delta $,
   \[\begin{array}{ll}
    &   \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (    \lambda    \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{21}}}}  .   \mathsf{let}  ~  \mathit{y}  \mathord{:}  \ottnt{T_{{\mathrm{11}}}}  \equal  \langle  \ottnt{T_{{\mathrm{21}}}}  \Rightarrow  \ottnt{T_{{\mathrm{11}}}}  \rangle   ^{ \ell }  \, \mathit{x}  ~ \ottliteralin ~  \langle  \ottnt{T_{{\mathrm{12}}}} \, [  \mathit{y}  \ottsym{/}  \mathit{x}  ]  \Rightarrow  \ottnt{T_{{\mathrm{22}}}}  \rangle   ^{ \ell }   \, \ottsym{(}  \ottnt{v_{{\mathrm{1}}}} \, \mathit{y}  \ottsym{)}   )   )  \, \ottnt{v'_{{\mathrm{1}}}}    \\   \simeq_{\mathtt{e} }   &    \ottnt{v_{{\mathrm{2}}}} \, \ottnt{v'_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T_{{\mathrm{22}}}} ;  \theta ;   \delta    [  \,  (  \ottnt{v'_{{\mathrm{1}}}}  ,  \ottnt{v'_{{\mathrm{2}}}}  ) /  \mathit{x}  \,  ]   .
     \end{array}\]

   Since $\Gamma  \vdash   \mathit{x} \mathord{:} \ottnt{T_{{\mathrm{11}}}} \rightarrow \ottnt{T_{{\mathrm{12}}}} $ and $\Gamma  \vdash   \mathit{x} \mathord{:} \ottnt{T_{{\mathrm{21}}}} \rightarrow \ottnt{T_{{\mathrm{22}}}} $,
   we have $\Gamma  \vdash  \ottnt{T_{{\mathrm{11}}}}$ and $\Gamma  \vdash  \ottnt{T_{{\mathrm{21}}}}$
   by their inversion.
   %
   Since $\Gamma  \vdash  \ottnt{T_{{\mathrm{21}}}}  \ottsym{<:}  \ottnt{T_{{\mathrm{11}}}}$ and $\Gamma  \vdash  \theta  \ottsym{;}  \delta$,
   we have
   \[
      \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T_{{\mathrm{21}}}}  \Rightarrow  \ottnt{T_{{\mathrm{11}}}}  \rangle   ^{ \ell }   )   )   \simeq_{\mathtt{v} }   \theta_{{\mathrm{2}}}  (   \delta_{{\mathrm{2}}}  (    \lambda    \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{21}}}}  .  \mathit{x}   )   )    \ottsym{:}   \ottnt{T_{{\mathrm{21}}}}  \rightarrow  \ottnt{T_{{\mathrm{11}}}} ;  \theta ;  \delta 
   \]
   by the IH.
   %
   Since $ \ottnt{v'_{{\mathrm{1}}}}  \simeq_{\mathtt{v} }  \ottnt{v'_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T_{{\mathrm{21}}}} ;  \theta ;  \delta $,
   we have
   \[
      \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T_{{\mathrm{21}}}}  \Rightarrow  \ottnt{T_{{\mathrm{11}}}}  \rangle   ^{ \ell }   )   )  \, \ottnt{v'_{{\mathrm{1}}}}  \simeq_{\mathtt{e} }  \ottnt{v'_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T_{{\mathrm{11}}}} ;  \theta ;  \delta .
   \]
   %
   By definition,
   there exists some $\ottnt{v''_{{\mathrm{1}}}}$ such that
   $ \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T_{{\mathrm{21}}}}  \Rightarrow  \ottnt{T_{{\mathrm{11}}}}  \rangle   ^{ \ell }   )   )  \, \ottnt{v'_{{\mathrm{1}}}}  \longrightarrow^{\ast}  \ottnt{v''_{{\mathrm{1}}}}$ and
   $ \ottnt{v''_{{\mathrm{1}}}}  \simeq_{\mathtt{v} }  \ottnt{v'_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T_{{\mathrm{11}}}} ;  \theta ;  \delta $.
   %
   Thus, it suffices to show that
   \[
      \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T_{{\mathrm{12}}}} \, [  \ottnt{v''_{{\mathrm{1}}}}  \ottsym{/}  \mathit{x}  ]  \Rightarrow  \ottnt{T_{{\mathrm{22}}}} \, [  \ottnt{v'_{{\mathrm{1}}}}  \ottsym{/}  \mathit{x}  ]  \rangle   ^{ \ell }   )   )  \, \ottsym{(}  \ottnt{v_{{\mathrm{1}}}} \, \ottnt{v''_{{\mathrm{1}}}}  \ottsym{)}  \simeq_{\mathtt{e} }  \ottnt{v_{{\mathrm{2}}}} \, \ottnt{v'_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T_{{\mathrm{22}}}} ;  \theta ;   \delta    [  \,  (  \ottnt{v'_{{\mathrm{1}}}}  ,  \ottnt{v'_{{\mathrm{2}}}}  ) /  \mathit{x}  \,  ]   .
   \]
   %
   Since $ \ottnt{v_{{\mathrm{1}}}}  \simeq_{\mathtt{v} }  \ottnt{v_{{\mathrm{2}}}}   \ottsym{:}    \mathit{x} \mathord{:} \ottnt{T_{{\mathrm{11}}}} \rightarrow \ottnt{T_{{\mathrm{12}}}}  ;  \theta ;  \delta $ and
   $ \ottnt{v''_{{\mathrm{1}}}}  \simeq_{\mathtt{v} }  \ottnt{v'_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T_{{\mathrm{11}}}} ;  \theta ;  \delta $,
   we have
   \[
     \ottnt{v_{{\mathrm{1}}}} \, \ottnt{v''_{{\mathrm{1}}}}  \simeq_{\mathtt{e} }  \ottnt{v_{{\mathrm{2}}}} \, \ottnt{v'_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T_{{\mathrm{12}}}} ;  \theta ;   \delta    [  \,  (  \ottnt{v''_{{\mathrm{1}}}}  ,  \ottnt{v'_{{\mathrm{2}}}}  ) /  \mathit{x}  \,  ]   .
   \]
   %
   If $\ottnt{v_{{\mathrm{1}}}} \, \ottnt{v''_{{\mathrm{1}}}}$ and $\ottnt{v_{{\mathrm{2}}}} \, \ottnt{v'_{{\mathrm{2}}}}$ raise blame, we finish.
   %
   Otherwise,
   $\ottnt{v_{{\mathrm{1}}}} \, \ottnt{v''_{{\mathrm{1}}}}  \longrightarrow^{\ast}  \ottnt{v'''_{{\mathrm{1}}}}$ and $\ottnt{v_{{\mathrm{2}}}} \, \ottnt{v'_{{\mathrm{2}}}}  \longrightarrow^{\ast}  \ottnt{v'''_{{\mathrm{2}}}}$
   for some $\ottnt{v'''_{{\mathrm{1}}}}$ and $\ottnt{v'''_{{\mathrm{2}}}}$, and it suffices to show that
   \[
      \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T_{{\mathrm{12}}}} \, [  \ottnt{v''_{{\mathrm{1}}}}  \ottsym{/}  \mathit{x}  ]  \Rightarrow  \ottnt{T_{{\mathrm{22}}}} \, [  \ottnt{v'_{{\mathrm{1}}}}  \ottsym{/}  \mathit{x}  ]  \rangle   ^{ \ell }   )   )  \, \ottnt{v'''_{{\mathrm{1}}}}  \simeq_{\mathtt{e} }  \ottnt{v'''_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T_{{\mathrm{22}}}} ;  \theta ;   \delta    [  \,  (  \ottnt{v'_{{\mathrm{1}}}}  ,  \ottnt{v'_{{\mathrm{2}}}}  ) /  \mathit{x}  \,  ]   .
   \]
   %
   We also have $ \ottnt{v'''_{{\mathrm{1}}}}  \simeq_{\mathtt{v} }  \ottnt{v'''_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T_{{\mathrm{12}}}} ;  \theta ;   \delta    [  \,  (  \ottnt{v''_{{\mathrm{1}}}}  ,  \ottnt{v'_{{\mathrm{2}}}}  ) /  \mathit{x}  \,  ]   $.
   %
   By $\alpha$-renaming $\mathit{x}$ in $\ottnt{T_{{\mathrm{12}}}}$ to $\mathit{y}$ {\iffull (\prop:ref{fh-lr-alpha-eq}) \fi} and
   the weakening (\prop:ref{fh-lr-val-ws(trel)}),
   \[
     \ottnt{v'''_{{\mathrm{1}}}}  \simeq_{\mathtt{v} }  \ottnt{v'''_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T_{{\mathrm{12}}}} \, [  \mathit{y}  \ottsym{/}  \mathit{x}  ] ;  \theta ;    \delta    [  \,  (  \ottnt{v'_{{\mathrm{1}}}}  ,  \ottnt{v'_{{\mathrm{2}}}}  ) /  \mathit{x}  \,  ]      [  \,  (  \ottnt{v''_{{\mathrm{1}}}}  ,  \ottnt{v'_{{\mathrm{2}}}}  ) /  \mathit{y}  \,  ]   .
   \]
   %
   Thus, it suffices to show that
   \begin{eqnarray}
    \begin{array}{ll}
    &   \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T_{{\mathrm{12}}}} \, [  \ottnt{v''_{{\mathrm{1}}}}  \ottsym{/}  \mathit{x}  ]  \Rightarrow  \ottnt{T_{{\mathrm{22}}}} \, [  \ottnt{v'_{{\mathrm{1}}}}  \ottsym{/}  \mathit{x}  ]  \rangle   ^{ \ell }   )   )     \\   \simeq_{\mathtt{v} }   &     \theta_{{\mathrm{2}}}  (   \delta_{{\mathrm{2}}}  (    \lambda    \mathit{z}  \mathord{:}  \ottnt{T'_{{\mathrm{12}}}}  .  \mathit{z}   )  \, [  \ottnt{v'_{{\mathrm{2}}}}  \ottsym{/}  \mathit{x}  ]  )    \ottsym{:}   \ottnt{T_{{\mathrm{12}}}} \, [  \mathit{y}  \ottsym{/}  \mathit{x}  ]  \rightarrow  \ottnt{T_{{\mathrm{22}}}} ;  \theta ;    \delta    [  \,  (  \ottnt{v'_{{\mathrm{1}}}}  ,  \ottnt{v'_{{\mathrm{2}}}}  ) /  \mathit{x}  \,  ]      [  \,  (  \ottnt{v''_{{\mathrm{1}}}}  ,  \ottnt{v'_{{\mathrm{2}}}}  ) /  \mathit{y}  \,  ]   .
     \label{req:fh-elim-upcast-aux-one}
    \end{array}
   \end{eqnarray}
   where $\ottnt{T'_{{\mathrm{12}}}}  \ottsym{=}  \ottnt{T_{{\mathrm{12}}}} \, [  \langle  \ottnt{T_{{\mathrm{21}}}}  \Rightarrow  \ottnt{T_{{\mathrm{11}}}}  \rangle   ^{ \ell }  \, \mathit{x}  \ottsym{/}  \mathit{x}  ]$.

   We first show
   \begin{equation}
    \begin{array}{ll}
     &   \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T_{{\mathrm{12}}}} \, [  \ottnt{v''_{{\mathrm{1}}}}  \ottsym{/}  \mathit{x}  ]  \Rightarrow  \ottnt{T_{{\mathrm{22}}}} \, [  \ottnt{v'_{{\mathrm{1}}}}  \ottsym{/}  \mathit{x}  ]  \rangle   ^{ \ell }   )   )     \\   \simeq_{\mathtt{v} }   &     \theta_{{\mathrm{2}}}  (   \delta_{{\mathrm{2}}}  (    \lambda    \mathit{z}  \mathord{:}  \ottnt{T'_{{\mathrm{12}}}}  .  \mathit{z}   )  \, [  \ottnt{v'_{{\mathrm{2}}}}  \ottsym{/}  \mathit{x}  ]  )    \ottsym{:}   \ottnt{T'_{{\mathrm{12}}}}  \rightarrow  \ottnt{T_{{\mathrm{22}}}} ;  \theta ;   \delta    [  \,  (  \ottnt{v'_{{\mathrm{1}}}}  ,  \ottnt{v'_{{\mathrm{2}}}}  ) /  \mathit{x}  \,  ]   
    \end{array}
     \label{eqn:fh-elim-upcast-aux-three}
   \end{equation}
   by applying Equivalence-Respecting (\prop:ref{fh-lr-comp-equiv-res}).
   %
   Since $\Gamma  \vdash   \mathit{x} \mathord{:} \ottnt{T_{{\mathrm{11}}}} \rightarrow \ottnt{T_{{\mathrm{12}}}} $ and $\Gamma  \vdash   \mathit{x} \mathord{:} \ottnt{T_{{\mathrm{21}}}} \rightarrow \ottnt{T_{{\mathrm{22}}}} $,
   we have $ \Gamma  ,  \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{11}}}}   \vdash  \ottnt{T_{{\mathrm{12}}}}$ and $ \Gamma  ,  \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{21}}}}   \vdash  \ottnt{T_{{\mathrm{22}}}}$.
   %
   By the typing weakening (\prop:ref{fh-weak-term}) and
   the term substitution (\prop:ref{fh-subst-term}),
   $ \Gamma  ,  \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{21}}}}   \vdash  \ottnt{T'_{{\mathrm{12}}}}$.
   %
   Since $\Gamma  \vdash  \theta  \ottsym{;}  \delta$ and $ \ottnt{v'_{{\mathrm{1}}}}  \simeq_{\mathtt{v} }  \ottnt{v'_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T_{{\mathrm{21}}}} ;  \theta ;  \delta $,
   we have $ \Gamma  ,  \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{21}}}}   \vdash  \theta  \ottsym{;}   \delta    [  \,  (  \ottnt{v'_{{\mathrm{1}}}}  ,  \ottnt{v'_{{\mathrm{2}}}}  ) /  \mathit{x}  \,  ]  $
   by the weakening of the logical relation (\prop:ref{fh-lr-val-ws(tctx)}).
   %
   Since $ \Gamma  ,  \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{21}}}}   \vdash  \ottnt{T_{{\mathrm{22}}}}$ and $ \Gamma  ,  \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{21}}}}   \vdash  \ottnt{T'_{{\mathrm{12}}}}  \ottsym{<:}  \ottnt{T_{{\mathrm{22}}}}$,
   we have
   \begin{equation}
      \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T'_{{\mathrm{12}}}}  \Rightarrow  \ottnt{T_{{\mathrm{22}}}}  \rangle   ^{ \ell }  \, [  \ottnt{v'_{{\mathrm{1}}}}  \ottsym{/}  \mathit{x}  ]  )   )   \simeq_{\mathtt{v} }   \theta_{{\mathrm{2}}}  (   \delta_{{\mathrm{2}}}  (    \lambda    \mathit{z}  \mathord{:}  \ottnt{T'_{{\mathrm{12}}}}  .  \mathit{z}   )  \, [  \ottnt{v'_{{\mathrm{2}}}}  \ottsym{/}  \mathit{x}  ]  )    \ottsym{:}   \ottnt{T'_{{\mathrm{12}}}}  \rightarrow  \ottnt{T_{{\mathrm{22}}}} ;  \theta ;   \delta    [  \,  (  \ottnt{v'_{{\mathrm{1}}}}  ,  \ottnt{v'_{{\mathrm{2}}}}  ) /  \mathit{x}  \,  ]   
     \label{eqn:fh-elim-upcast-aux-one}
   \end{equation}
   by the IH.
   %
   Furthermore, since $ \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T_{{\mathrm{21}}}}  \Rightarrow  \ottnt{T_{{\mathrm{11}}}}  \rangle   ^{ \ell }   )   )  \, \ottnt{v'_{{\mathrm{1}}}}  \longrightarrow^{\ast}  \ottnt{v''_{{\mathrm{1}}}}$,
   we can show
   \begin{equation}
    \begin{array}{ll}
     & \emptyset  \vdash   \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T_{{\mathrm{12}}}} \, [  \ottnt{v''_{{\mathrm{1}}}}  \ottsym{/}  \mathit{x}  ]  \Rightarrow  \ottnt{T_{{\mathrm{22}}}} \, [  \ottnt{v'_{{\mathrm{1}}}}  \ottsym{/}  \mathit{x}  ]  \rangle   ^{ \ell }   )   )  \,  \\  \, =_\mathsf{ciu} \,  &  \,  \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T'_{{\mathrm{12}}}}  \Rightarrow  \ottnt{T_{{\mathrm{22}}}}  \rangle   ^{ \ell }   )  \, [  \ottnt{v'_{{\mathrm{1}}}}  \ottsym{/}  \mathit{x}  ]  )   \ottsym{:}   \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \ottnt{T'_{{\mathrm{12}}}}  \rightarrow  \ottnt{T_{{\mathrm{22}}}}  )  \, [  \ottnt{v'_{{\mathrm{1}}}}  \ottsym{/}  \mathit{x}  ]  ) 
    \end{array}
    \label{eqn:fh-elim-upcast-aux-two}
   \end{equation}
   %
   by using Cotermination.
   %
   From (\ref{eqn:fh-elim-upcast-aux-one}) and (\ref{eqn:fh-elim-upcast-aux-two}),
   Equivalence-Respecting derives (\ref{eqn:fh-elim-upcast-aux-three}).

   We show (\ref{req:fh-elim-upcast-aux-one})
   by applying (\ref{eqn:fh-elim-upcast-aux-three}) to Term Compositionality (\prop:ref{fh-lr-term-comp}).
   %
   Since $\ottnt{T'_{{\mathrm{12}}}}  \ottsym{=}  \ottnt{T_{{\mathrm{12}}}} \, [  \langle  \ottnt{T_{{\mathrm{21}}}}  \Rightarrow  \ottnt{T_{{\mathrm{11}}}}  \rangle   ^{ \ell }  \, \mathit{x}  \ottsym{/}  \mathit{x}  ]  \ottsym{=}  \ottnt{T_{{\mathrm{12}}}} \, [  \mathit{y}  \ottsym{/}  \mathit{x}  ] \, [  \langle  \ottnt{T_{{\mathrm{21}}}}  \Rightarrow  \ottnt{T_{{\mathrm{11}}}}  \rangle   ^{ \ell }  \, \mathit{x}  \ottsym{/}  \mathit{y}  ]$,
   it suffices to show that
   \begin{enumerate}
    \item \label{req:fh-elim-upcast-aux-Gself}
          $  \Gamma  ,  \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{21}}}}   ,  \mathit{y}  \mathord{:}  \ottnt{T_{{\mathrm{11}}}} $ is self-related,
    \item \label{req:fh-elim-upcast-aux-T12self}
          $   \Gamma  ,  \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{21}}}}   ,  \mathit{y}  \mathord{:}  \ottnt{T_{{\mathrm{11}}}}  \vdash \ottnt{T_{{\mathrm{12}}}} \, [  \mathit{y}  \ottsym{/}  \mathit{x}  ]  \mathrel{ \simeq }  \ottnt{T_{{\mathrm{12}}}} \, [  \mathit{y}  \ottsym{/}  \mathit{x}  ]  : \ast $,
    \item \label{req:fh-elim-upcast-aux-subst}
          $  \Gamma  ,  \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{21}}}}   ,  \mathit{y}  \mathord{:}  \ottnt{T_{{\mathrm{11}}}}   \vdash  \theta  \ottsym{;}    \delta    [  \,  (  \ottnt{v'_{{\mathrm{1}}}}  ,  \ottnt{v'_{{\mathrm{2}}}}  ) /  \mathit{x}  \,  ]      [  \,  (  \ottnt{v''_{{\mathrm{1}}}}  ,  \ottnt{v'_{{\mathrm{2}}}}  ) /  \mathit{y}  \,  ]  $,
    % \item \label{req:fh-elim-upcast-aux-v1}
    %       $ \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T_{{\mathrm{21}}}}  \Rightarrow  \ottnt{T_{{\mathrm{11}}}}  \rangle   ^{ \ell }   )   )  \, \ottnt{v'_{{\mathrm{1}}}}  \longrightarrow^{\ast}  \ottnt{v''_{{\mathrm{1}}}}$,
    \item \label{req:fh-elim-upcast-aux-v2}
          $ \theta_{{\mathrm{2}}}  (   \delta_{{\mathrm{2}}}  (  \langle  \ottnt{T_{{\mathrm{21}}}}  \Rightarrow  \ottnt{T_{{\mathrm{11}}}}  \rangle   ^{ \ell }   )   )  \, \ottnt{v'_{{\mathrm{2}}}}  \longrightarrow^{\ast}  \ottnt{v''_{{\mathrm{2}}}}$ and
          $ \ottnt{v''_{{\mathrm{1}}}}  \simeq_{\mathtt{v} }  \ottnt{v''_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T_{{\mathrm{11}}}} ;  \theta ;   \delta    [  \,  (  \ottnt{v'_{{\mathrm{1}}}}  ,  \ottnt{v'_{{\mathrm{2}}}}  ) /  \mathit{x}  \,  ]   $
          for some $\ottnt{v''_{{\mathrm{2}}}}$.
   \end{enumerate}

   Since $ \Gamma  ,  \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{11}}}}   \vdash  \ottnt{T_{{\mathrm{12}}}}$, we have
   $  \Gamma  ,  \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{21}}}}   ,  \mathit{y}  \mathord{:}  \ottnt{T_{{\mathrm{11}}}}   \vdash  \ottnt{T_{{\mathrm{12}}}} \, [  \mathit{y}  \ottsym{/}  \mathit{x}  ]$.
   %
   By Parametricity (\prop:ref{fh-lr-param}), we have
   (\ref{req:fh-elim-upcast-aux-Gself}) and
   (\ref{req:fh-elim-upcast-aux-T12self}).

   Since $\Gamma  \vdash  \theta  \ottsym{;}  \delta$ and
   $ \ottnt{v''_{{\mathrm{1}}}}  \simeq_{\mathtt{v} }  \ottnt{v'_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T_{{\mathrm{11}}}} ;  \theta ;  \delta $ and
   $ \ottnt{v'_{{\mathrm{1}}}}  \simeq_{\mathtt{v} }  \ottnt{v'_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T_{{\mathrm{21}}}} ;  \theta ;  \delta $,
   we have (\ref{req:fh-elim-upcast-aux-subst})
   by the weakening (\prop:ref{fh-lr-val-ws(tctx)}).

   Since $\Gamma  \vdash  \theta  \ottsym{;}  \delta$ and
   $ \ottnt{v'_{{\mathrm{1}}}}  \simeq_{\mathtt{v} }  \ottnt{v'_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T_{{\mathrm{21}}}} ;  \theta ;  \delta $,
   we have $ \Gamma  ,  \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{21}}}}   \vdash  \theta  \ottsym{;}   \delta    [  \,  (  \ottnt{v'_{{\mathrm{1}}}}  ,  \ottnt{v'_{{\mathrm{2}}}}  ) /  \mathit{x}  \,  ]  $.
   %
   Since $ \Gamma  ,  \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{21}}}}   \vdash  \langle  \ottnt{T_{{\mathrm{21}}}}  \Rightarrow  \ottnt{T_{{\mathrm{11}}}}  \rangle   ^{ \ell }  \, \mathit{x}  \ottsym{:}  \ottnt{T_{{\mathrm{11}}}}$,
   we have $ \Gamma  ,  \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{21}}}}   \vdash  \langle  \ottnt{T_{{\mathrm{21}}}}  \Rightarrow  \ottnt{T_{{\mathrm{11}}}}  \rangle   ^{ \ell }  \, \mathit{x} \,  \mathrel{ \simeq }  \, \langle  \ottnt{T_{{\mathrm{21}}}}  \Rightarrow  \ottnt{T_{{\mathrm{11}}}}  \rangle   ^{ \ell }  \, \mathit{x}  \ottsym{:}  \ottnt{T_{{\mathrm{11}}}}$
   by Parametricity (\prop:ref{fh-lr-param}).
   %
   Thus, by definition,
   \[
      \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T_{{\mathrm{21}}}}  \Rightarrow  \ottnt{T_{{\mathrm{11}}}}  \rangle   ^{ \ell }   )   )  \, \ottnt{v'_{{\mathrm{1}}}}  \simeq_{\mathtt{e} }   \theta_{{\mathrm{2}}}  (   \delta_{{\mathrm{2}}}  (  \langle  \ottnt{T_{{\mathrm{21}}}}  \Rightarrow  \ottnt{T_{{\mathrm{11}}}}  \rangle   ^{ \ell }   )   )  \, \ottnt{v'_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T_{{\mathrm{11}}}} ;  \theta ;   \delta    [  \,  (  \ottnt{v'_{{\mathrm{1}}}}  ,  \ottnt{v'_{{\mathrm{2}}}}  ) /  \mathit{x}  \,  ]   .
   \]
   %
   Since $ \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T_{{\mathrm{21}}}}  \Rightarrow  \ottnt{T_{{\mathrm{11}}}}  \rangle   ^{ \ell }   )   )  \, \ottnt{v'_{{\mathrm{1}}}}  \longrightarrow^{\ast}  \ottnt{v''_{{\mathrm{1}}}}$,
   we have (\ref{req:fh-elim-upcast-aux-v2}).

  \case \Sub{Forall}: By the IH.
  \case \Sub{RefineL}: By the IH.
   %
   {\iffull
   %
   We are given $\Gamma  \vdash   \{  \mathit{x}  \mathord{:}  \ottnt{T'_{{\mathrm{1}}}}   \mathop{\mid}   \ottnt{e'_{{\mathrm{1}}}}  \}   \ottsym{<:}  \ottnt{T_{{\mathrm{2}}}}$.
   %
   By inversion, $\Gamma  \vdash  \ottnt{T'_{{\mathrm{1}}}}  \ottsym{<:}  \ottnt{T_{{\mathrm{2}}}}$.
   %
   By \E{Red}/\R{Forget},
   $ \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle   \{  \mathit{x}  \mathord{:}  \ottnt{T'_{{\mathrm{1}}}}   \mathop{\mid}   \ottnt{e'_{{\mathrm{1}}}}  \}   \Rightarrow  \ottnt{T_{{\mathrm{2}}}}  \rangle   ^{ \ell }   )   )  \, \ottnt{v_{{\mathrm{1}}}}  \longrightarrow   \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T'_{{\mathrm{1}}}}  \Rightarrow  \ottnt{T_{{\mathrm{2}}}}  \rangle   ^{ \ell }   )   )  \, \ottnt{v_{{\mathrm{1}}}}$.
   %
   Thus, it suffices to show that
   \[
      \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T'_{{\mathrm{1}}}}  \Rightarrow  \ottnt{T_{{\mathrm{2}}}}  \rangle   ^{ \ell }   )   )  \, \ottnt{v_{{\mathrm{1}}}}  \simeq_{\mathtt{e} }  \ottnt{v_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T_{{\mathrm{2}}}} ;  \theta ;  \delta .
   \]
   %
   It can be proven straightforwardly by the IH.
   %
   \fi}

  \case \Sub{RefineR}:
   %
   We are given $\Gamma  \vdash  \ottnt{T_{{\mathrm{1}}}}  \ottsym{<:}   \{  \mathit{x}  \mathord{:}  \ottnt{T'_{{\mathrm{2}}}}   \mathop{\mid}   \ottnt{e'_{{\mathrm{2}}}}  \} $.
   %
   By inversion,
   $\Gamma  \vdash  \ottnt{T_{{\mathrm{1}}}}  \ottsym{<:}  \ottnt{T'_{{\mathrm{2}}}}$ and $ \Gamma  ,  \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{1}}}}   \models  \ottnt{e'_{{\mathrm{2}}}} \, [  \langle  \ottnt{T_{{\mathrm{1}}}}  \Rightarrow  \ottnt{T'_{{\mathrm{2}}}}  \rangle   ^{ \ell }  \, \mathit{x}  \ottsym{/}  \mathit{x}  ]$.
   %
   By \E{Red}/\R{Forget},
   \[
     \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T_{{\mathrm{1}}}}  \Rightarrow   \{  \mathit{x}  \mathord{:}  \ottnt{T'_{{\mathrm{2}}}}   \mathop{\mid}   \ottnt{e'_{{\mathrm{2}}}}  \}   \rangle   ^{ \ell }   )   )  \, \ottnt{v_{{\mathrm{1}}}}  \longrightarrow^{\ast}  \langle   \mathit{unref}  (   \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \ottnt{T_{{\mathrm{1}}}}  )   )   )   \Rightarrow   \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (   \{  \mathit{x}  \mathord{:}  \ottnt{T'_{{\mathrm{2}}}}   \mathop{\mid}   \ottnt{e'_{{\mathrm{2}}}}  \}   )   )   \rangle   ^{ \ell }  \, \ottnt{v_{{\mathrm{1}}}}.
   \]
   %
   By \E{Red}/\R{PreCheck},
   \[\begin{array}{ll}
    & \langle   \mathit{unref}  (   \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \ottnt{T_{{\mathrm{1}}}}  )   )   )   \Rightarrow   \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (   \{  \mathit{x}  \mathord{:}  \ottnt{T'_{{\mathrm{2}}}}   \mathop{\mid}   \ottnt{e'_{{\mathrm{2}}}}  \}   )   )   \rangle   ^{ \ell }  \, \ottnt{v_{{\mathrm{1}}}} \\
     \longrightarrow  &
       \langle\!\langle  \,  \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (   \{  \mathit{x}  \mathord{:}  \ottnt{T'_{{\mathrm{2}}}}   \mathop{\mid}   \ottnt{e'_{{\mathrm{2}}}}  \}   )   )   \ottsym{,}  \langle   \mathit{unref}  (   \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \ottnt{T_{{\mathrm{1}}}}  )   )   )   \Rightarrow   \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \ottnt{T'_{{\mathrm{2}}}}  )   )   \rangle   ^{ \ell }  \, \ottnt{v_{{\mathrm{1}}}} \,  \rangle\!\rangle  \,  ^{ \ell } .
     \end{array}\]
   %
   Thus, it suffices to show that
   \[
      \langle\!\langle  \,  \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (   \{  \mathit{x}  \mathord{:}  \ottnt{T'_{{\mathrm{2}}}}   \mathop{\mid}   \ottnt{e'_{{\mathrm{2}}}}  \}   )   )   \ottsym{,}  \langle   \mathit{unref}  (   \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \ottnt{T_{{\mathrm{1}}}}  )   )   )   \Rightarrow   \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \ottnt{T'_{{\mathrm{2}}}}  )   )   \rangle   ^{ \ell }  \, \ottnt{v_{{\mathrm{1}}}} \,  \rangle\!\rangle  \,  ^{ \ell }   \simeq_{\mathtt{e} }  \ottnt{v_{{\mathrm{2}}}}   \ottsym{:}    \{  \mathit{x}  \mathord{:}  \ottnt{T'_{{\mathrm{2}}}}   \mathop{\mid}   \ottnt{e'_{{\mathrm{2}}}}  \}  ;  \theta ;  \delta .
   \]

   Since $\Gamma  \vdash   \{  \mathit{x}  \mathord{:}  \ottnt{T'_{{\mathrm{2}}}}   \mathop{\mid}   \ottnt{e'_{{\mathrm{2}}}}  \} $,
   we have $\Gamma  \vdash  \ottnt{T'_{{\mathrm{2}}}}$ by its inversion.
   %
   Thus, by the IH,
   \[
      \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T_{{\mathrm{1}}}}  \Rightarrow  \ottnt{T'_{{\mathrm{2}}}}  \rangle   ^{ \ell }   )   )   \simeq_{\mathtt{v} }   \theta_{{\mathrm{2}}}  (   \delta_{{\mathrm{2}}}  (    \lambda    \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{1}}}}  .  \mathit{x}   )   )    \ottsym{:}   \ottnt{T_{{\mathrm{1}}}}  \rightarrow  \ottnt{T'_{{\mathrm{2}}}} ;  \theta ;  \delta .
   \]
   %
   Since $ \ottnt{v_{{\mathrm{1}}}}  \simeq_{\mathtt{v} }  \ottnt{v_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T_{{\mathrm{1}}}} ;  \theta ;  \delta $,
   we have
   \[
      \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T_{{\mathrm{1}}}}  \Rightarrow  \ottnt{T'_{{\mathrm{2}}}}  \rangle   ^{ \ell }   )   )  \, \ottnt{v_{{\mathrm{1}}}}  \simeq_{\mathtt{e} }  \ottnt{v_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T'_{{\mathrm{2}}}} ;  \theta ;  \delta .
   \]
   %
   Since
   $ \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T_{{\mathrm{1}}}}  \Rightarrow  \ottnt{T'_{{\mathrm{2}}}}  \rangle   ^{ \ell }   )   )  \, \ottnt{v_{{\mathrm{1}}}}  \longrightarrow^{\ast}  \langle   \mathit{unref}  (   \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \ottnt{T_{{\mathrm{1}}}}  )   )   )   \Rightarrow   \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \ottnt{T'_{{\mathrm{2}}}}  )   )   \rangle   ^{ \ell }  \, \ottnt{v_{{\mathrm{1}}}}$,
   we have
   \[
     \langle   \mathit{unref}  (   \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \ottnt{T_{{\mathrm{1}}}}  )   )   )   \Rightarrow   \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \ottnt{T'_{{\mathrm{2}}}}  )   )   \rangle   ^{ \ell }  \, \ottnt{v_{{\mathrm{1}}}}  \simeq_{\mathtt{e} }  \ottnt{v_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T'_{{\mathrm{2}}}} ;  \theta ;  \delta .
   \]
   %
   By definition,
   there exists some $\ottnt{v'_{{\mathrm{1}}}}$ such that
   $\langle   \mathit{unref}  (   \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \ottnt{T_{{\mathrm{1}}}}  )   )   )   \Rightarrow   \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \ottnt{T'_{{\mathrm{2}}}}  )   )   \rangle   ^{ \ell }  \, \ottnt{v_{{\mathrm{1}}}}  \longrightarrow^{\ast}  \ottnt{v'_{{\mathrm{1}}}}$
   and
   $ \ottnt{v'_{{\mathrm{1}}}}  \simeq_{\mathtt{v} }  \ottnt{v_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T'_{{\mathrm{2}}}} ;  \theta ;  \delta $.
   %
   Thus, it suffices to show that
   \[
      \langle\!\langle  \,  \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (   \{  \mathit{x}  \mathord{:}  \ottnt{T'_{{\mathrm{2}}}}   \mathop{\mid}   \ottnt{e'_{{\mathrm{2}}}}  \}   )   )   \ottsym{,}  \ottnt{v'_{{\mathrm{1}}}} \,  \rangle\!\rangle  \,  ^{ \ell }   \simeq_{\mathtt{e} }  \ottnt{v_{{\mathrm{2}}}}   \ottsym{:}    \{  \mathit{x}  \mathord{:}  \ottnt{T'_{{\mathrm{2}}}}   \mathop{\mid}   \ottnt{e'_{{\mathrm{2}}}}  \}  ;  \theta ;  \delta .
   \]

   Since
   $\Gamma  \vdash  \theta  \ottsym{;}  \delta$ and $ \ottnt{v_{{\mathrm{1}}}}  \simeq_{\mathtt{v} }  \ottnt{v_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T_{{\mathrm{1}}}} ;  \theta ;  \delta $,
   we have $ \Gamma  ,  \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{1}}}}   \vdash   \theta_{{\mathrm{1}}} \circ \delta_{{\mathrm{1}}}   [  \ottnt{v_{{\mathrm{1}}}}  \ottsym{/}  \mathit{x}  ]$.
   %
   Since $ \Gamma  ,  \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{1}}}}   \models  \ottnt{e'_{{\mathrm{2}}}} \, [  \langle  \ottnt{T_{{\mathrm{1}}}}  \Rightarrow  \ottnt{T'_{{\mathrm{2}}}}  \rangle   ^{ \ell }  \, \mathit{x}  \ottsym{/}  \mathit{x}  ]$,
   we have $ \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \ottnt{e'_{{\mathrm{2}}}} \, [  \langle  \ottnt{T_{{\mathrm{1}}}}  \Rightarrow  \ottnt{T'_{{\mathrm{2}}}}  \rangle   ^{ \ell }  \, \ottnt{v_{{\mathrm{1}}}}  \ottsym{/}  \mathit{x}  ]  )   )   \longrightarrow^{\ast}   \mathsf{true} $.
   %
   Since $ \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \langle  \ottnt{T_{{\mathrm{1}}}}  \Rightarrow  \ottnt{T'_{{\mathrm{2}}}}  \rangle   ^{ \ell }   )   )  \, \ottnt{v_{{\mathrm{1}}}}  \longrightarrow^{\ast}  \ottnt{v'_{{\mathrm{1}}}}$,
   we have $ \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \ottnt{e'_{{\mathrm{2}}}} \, [  \ottnt{v'_{{\mathrm{1}}}}  \ottsym{/}  \mathit{x}  ]  )   )   \longrightarrow^{\ast}   \mathsf{true} $
   by Cotermination (\prop:ref{fh-coterm-true}).
   %
   Thus,
   $ \langle\!\langle  \,  \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (   \{  \mathit{x}  \mathord{:}  \ottnt{T'_{{\mathrm{2}}}}   \mathop{\mid}   \ottnt{e'_{{\mathrm{2}}}}  \}   )   )   \ottsym{,}  \ottnt{v'_{{\mathrm{1}}}} \,  \rangle\!\rangle  \,  ^{ \ell }   \longrightarrow^{\ast}  \ottnt{v'_{{\mathrm{1}}}}$
   (by \R{Check} and \R{OK}), and so
   it suffices to show that
   \[
     \ottnt{v'_{{\mathrm{1}}}}  \simeq_{\mathtt{v} }  \ottnt{v_{{\mathrm{2}}}}   \ottsym{:}    \{  \mathit{x}  \mathord{:}  \ottnt{T'_{{\mathrm{2}}}}   \mathop{\mid}   \ottnt{e'_{{\mathrm{2}}}}  \}  ;  \theta ;  \delta .
   \]
   %
   Since
   $ \ottnt{v'_{{\mathrm{1}}}}  \simeq_{\mathtt{v} }  \ottnt{v_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T'_{{\mathrm{2}}}} ;  \theta ;  \delta $ and
   $ \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \ottnt{e'_{{\mathrm{2}}}} \, [  \ottnt{v'_{{\mathrm{1}}}}  \ottsym{/}  \mathit{x}  ]  )   )   \longrightarrow^{\ast}   \mathsf{true} $,
   it suffices to show that
   \[
     \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \ottnt{e'_{{\mathrm{2}}}} \, [  \ottnt{v_{{\mathrm{2}}}}  \ottsym{/}  \mathit{x}  ]  )   )   \longrightarrow^{\ast}   \mathsf{true} .
   \]
   %
   Since $\Gamma  \vdash   \{  \mathit{x}  \mathord{:}  \ottnt{T'_{{\mathrm{2}}}}   \mathop{\mid}   \ottnt{e'_{{\mathrm{2}}}}  \} $,
   we have $ \Gamma  ,  \mathit{x}  \mathord{:}  \ottnt{T'_{{\mathrm{2}}}}   \vdash  \ottnt{e'_{{\mathrm{2}}}}  \ottsym{:}   \mathsf{Bool} $ by its inversion.
   %
   By Parametricity (\prop:ref{fh-lr-param}),
   $ \Gamma  ,  \mathit{x}  \mathord{:}  \ottnt{T'_{{\mathrm{2}}}}   \vdash  \ottnt{e'_{{\mathrm{2}}}} \,  \mathrel{ \simeq }  \, \ottnt{e'_{{\mathrm{2}}}}  \ottsym{:}   \mathsf{Bool} $.
   %
   Since $\Gamma  \vdash  \theta  \ottsym{;}  \delta$ and $ \ottnt{v'_{{\mathrm{1}}}}  \simeq_{\mathtt{v} }  \ottnt{v_{{\mathrm{2}}}}   \ottsym{:}   \ottnt{T'_{{\mathrm{2}}}} ;  \theta ;  \delta $,
   we have $ \Gamma  ,  \mathit{x}  \mathord{:}  \ottnt{T'_{{\mathrm{2}}}}   \vdash  \theta  \ottsym{;}   \delta    [  \,  (  \ottnt{v'_{{\mathrm{1}}}}  ,  \ottnt{v_{{\mathrm{2}}}}  ) /  \mathit{x}  \,  ]  $.
   %
   Thus,
   \[
      \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \ottnt{e'_{{\mathrm{2}}}} \, [  \ottnt{v'_{{\mathrm{1}}}}  \ottsym{/}  \mathit{x}  ]  )   )   \simeq_{\mathtt{e} }   \theta_{{\mathrm{2}}}  (   \delta_{{\mathrm{2}}}  (  \ottnt{e'_{{\mathrm{2}}}} \, [  \ottnt{v_{{\mathrm{2}}}}  \ottsym{/}  \mathit{x}  ]  )   )    \ottsym{:}    \mathsf{Bool}  ;  \theta ;   \delta    [  \,  (  \ottnt{v'_{{\mathrm{1}}}}  ,  \ottnt{v_{{\mathrm{2}}}}  ) /  \mathit{x}  \,  ]   .
   \]
   %
   Since the term on the left-hand side evaluates to $ \mathsf{true} $,
   we have $ \theta_{{\mathrm{1}}}  (   \delta_{{\mathrm{1}}}  (  \ottnt{e'_{{\mathrm{2}}}} \, [  \ottnt{v_{{\mathrm{2}}}}  \ottsym{/}  \mathit{x}  ]  )   )   \longrightarrow^{\ast}   \mathsf{true} $ by definition.
 \end{itemize}
\end{prop}

\begin{prop}[type=thm,name=Upcast Elimination]{elim-upcast}
 If $\Gamma  \vdash  \ottnt{T_{{\mathrm{1}}}}$ and $\Gamma  \vdash  \ottnt{T_{{\mathrm{2}}}}$ and $\Gamma  \vdash  \ottnt{T_{{\mathrm{1}}}}  \ottsym{<:}  \ottnt{T_{{\mathrm{2}}}}$,
 then $\Gamma  \vdash  \langle  \ottnt{T_{{\mathrm{1}}}}  \Rightarrow  \ottnt{T_{{\mathrm{2}}}}  \rangle   ^{ \ell }  \, =_\mathsf{ctx} \, \ottsym{(}    \lambda    \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{1}}}}  .  \mathit{x}   \ottsym{)}  \ottsym{:}  \ottnt{T_{{\mathrm{1}}}}  \rightarrow  \ottnt{T_{{\mathrm{2}}}}$.

 \proof

 By \prop:ref{fh-elim-upcast-aux}, $\Gamma  \vdash  \langle  \ottnt{T_{{\mathrm{1}}}}  \Rightarrow  \ottnt{T_{{\mathrm{2}}}}  \rangle   ^{ \ell }  \,  \mathrel{ \simeq }  \, \ottsym{(}    \lambda    \mathit{x}  \mathord{:}  \ottnt{T_{{\mathrm{1}}}}  .  \mathit{x}   \ottsym{)}  \ottsym{:}  \ottnt{T_{{\mathrm{1}}}}  \rightarrow  \ottnt{T_{{\mathrm{2}}}}$.
 %
 By soundness of the logical relation (\refthm{fh-lr-sound}), we finish.
\end{prop}

